Risk-Averse Decision Making Under Uncertainty

A large class of decision making under uncertainty problems can be described via Markov decision processes (MDPs) or partially observable MDPs (POMDPs), with application to artificial intelligence and operations research, among others. Traditionally, policy synthesis techniques are proposed such that a total expected cost or reward is minimized or maximized. However, optimality in the total expected cost sense is only reasonable if system behavior in the large number of runs is of interest, which has limited the use of such policies in practical mission-critical scenarios, wherein large deviations from the expected behavior may lead to mission failure. In this paper, we consider the problem of designing policies for MDPs and POMDPs with objectives and constraints in terms of dynamic coherent risk measures, which we refer to as the constrained risk-averse problem. For MDPs, we reformulate the problem into a infsup problem via the Lagrangian framework and propose an optimization-based method to synthesize Markovian policies. For MDPs, we demonstrate that the formulated optimization problems are in the form of difference convex programs (DCPs) and can be solved by the disciplined convex-concave programming (DCCP) framework. We show that these results generalize linear programs for constrained MDPs with total discounted expected costs and constraints. For POMDPs, we show that, if the coherent risk measures can be defined as a Markov risk transition mapping, an infinite-dimensional optimization can be used to design Markovian belief-based policies. For stochastic finite-state controllers (FSCs), we show that the latter optimization simplifies to a (finite-dimensional) DCP and can be solved by the DCCP framework. We incorporate these DCPs in a policy iteration algorithm to design risk-averse FSCs for POMDPs.

==> Risk-Averse Decision Making Under Uncertainty (1)/walkingExample.tex <==

In previous section, we used a numerical example to elucidate our proposed methodology. In the following, we demonstrate the application of risk barrier functions for bipedal walking. A linear discrete dynamics is used to approximate (with uncertainties) the actual step-to-step (S2S) dynamics of the robot walking for step planning. More details about the step planning can be found in \cite{xiong2021inReview}. Here we briefly describe the stepping controller, the problem setups, and the applications of risk barrier functions.
  
\subsubsection{Stepping Controller for Walking}
The walking of the robot is modeled as a hybrid dynamical system which is composed by continuous dynamics and discrete transitions \cite{grizzle2014models}. We use the general two-domain hybrid system of walking; the continuous dynamics is thus composed by a single support phase (SSP) and a double support phase, and the discrete transitions are between the SSP and DSP. We apply the Hybrid-Linear Inverted Pendulum (H-LIP) based approach in \cite{xiong} to synthesis and stabilize walking gait. The walking behavior, i.e., the horizontal center of mass (COM) trajectory, is controlled by the step size based on the step-to-step dynamics approximation via the H-LIP. The S2S dynamics of the robot is 
\begin{equation}
\label{eq:S2S}
    \mathbf{x}_{k+1} = A \mathbf{x}_k + B u_k +w 
\end{equation}
where $\mathbf{x}$ is the discrete horizontal COM state at the pre-impact event, $u$ is the step size on the robot, $A$ and $B$ are the matrices of the linear S2S dynamics of the H-LIP, and $w$ is the difference of the S2S dynamics between the robot and the H-LIP.  
The step size on the robot is calculated based on the H-LIP stepping:
\begin{equation}
    u = u^\text{H-LIP} + K (\mathbf{x} -\mathbf{x}^\text{H-LIP}  )
\end{equation}
which makes sure that the robot state is close to the state of the H-LIP $\mathbf{x}^\text{H-LIP}$; $K$ is a feedback gain to make $A+BK$ stable. In the later, we use the disturbed linear dynamics in Eq. \eqref{eq:S2S} to plan for walking behaviors on the H-LIP and then apply the H-LIP stepping to realize the walking on the robot. Barrier functions are synthesized for guaranteeing safety on the robot walking. 


\subsubsection{Problem Definition}
We consider the following scenarios of controlling the robot. 
  
\noindent{\textbf{Reaching a Target Region:}} We consider a case where the robot should walk to reach to a target square region, which is defined via four barrier functions. Without the barrier function, the robot is supposed to walking in place with not horizontal velocity. By integrating the barrier function in the planning via the H-LIP based controller, the robot walks to the target region and stays inside.

  
\noindent{\textbf{Path Tracking with Obstacle Avoidance:}} We also consider a case where the robot walks to follow a path with obstacles along the path. The barrier functions are designed to represent collision-free regions in the space. Here we demonstrate the walking without and with the barrier functions. Without the barrier functions in the controller, the robot precisely follows the path but then inevitably collides with the obstacles. With the barrier functions, the robot follows the path when it can and avoids obstacles when it has to.


==> walkingExample.tex <==

In previous section, we used a numerical example to elucidate our proposed methodology. In the following, we demonstrate the application of risk barrier functions for bipedal walking. A linear discrete dynamics is used to approximate (with uncertainties) the actual step-to-step (S2S) dynamics of the robot walking for step planning. More details about the step planning can be found in \cite{xiong2021inReview}. Here we briefly describe the stepping controller, the problem setups, and the applications of risk barrier functions.
  
\subsubsection{Stepping Controller for Walking}
The walking of the robot is modeled as a hybrid dynamical system which is composed by continuous dynamics and discrete transitions \cite{grizzle2014models}. We use the general two-domain hybrid system of walking; the continuous dynamics is thus composed by a single support phase (SSP) and a double support phase, and the discrete transitions are between the SSP and DSP. We apply the Hybrid-Linear Inverted Pendulum (H-LIP) based approach in \cite{xiong} to synthesis and stabilize walking gait. The walking behavior, i.e., the horizontal center of mass (COM) trajectory, is controlled by the step size based on the step-to-step dynamics approximation via the H-LIP. The S2S dynamics of the robot is 
\begin{equation}
\label{eq:S2S}
    \mathbf{x}_{k+1} = A \mathbf{x}_k + B u_k +w 
\end{equation}
where $\mathbf{x}$ is the discrete horizontal COM state at the pre-impact event, $u$ is the step size on the robot, $A$ and $B$ are the matrices of the linear S2S dynamics of the H-LIP, and $w$ is the difference of the S2S dynamics between the robot and the H-LIP.  
The step size on the robot is calculated based on the H-LIP stepping:
\begin{equation}
    u = u^\text{H-LIP} + K (\mathbf{x} -\mathbf{x}^\text{H-LIP}  )
\end{equation}
which makes sure that the robot state is close to the state of the H-LIP $\mathbf{x}^\text{H-LIP}$; $K$ is a feedback gain to make $A+BK$ stable. In the later, we use the disturbed linear dynamics in Eq. \eqref{eq:S2S} to plan for walking behaviors on the H-LIP and then apply the H-LIP stepping to realize the walking on the robot. Barrier functions are synthesized for guaranteeing safety on the robot walking. 


\subsubsection{Problem Definition}
We consider the following scenarios of controlling the robot. 
  
\noindent{\textbf{Reaching a Target Region:}} We consider a case where the robot should walk to reach to a target square region, which is defined via four barrier functions. Without the barrier function, the robot is supposed to walking in place with not horizontal velocity. By integrating the barrier function in the planning via the H-LIP based controller, the robot walks to the target region and stays inside.

  
\noindent{\textbf{Path Tracking with Obstacle Avoidance:}} We also consider a case where the robot walks to follow a path with obstacles along the path. The barrier functions are designed to represent collision-free regions in the space. Here we demonstrate the walking without and with the barrier functions. Without the barrier functions in the controller, the robot precisely follows the path but then inevitably collides with the obstacles. With the barrier functions, the robot follows the path when it can and avoids obstacles when it has to.

